Recursive Think-Answer Process for LLMs and VLMs

Think-Answer reasoners such as DeepSeek-R1 have made notable progress by leveraging interpretable internal reasoning. However, despite the frequent presence of self-reflective cues like "Oops!", they remain vulnerable to output errors during single-pass inference. To address this limitation, we propose an efficient Recursive Think-Answer Process (R-TAP) that enables models to engage in iterative reasoning cycles and generate more accurate answers, going beyond conventional single-pass approaches. Central to this approach is a confidence generator that evaluates the certainty of model responses and guides subsequent improvements. By incorporating two complementary rewards-Recursively Confidence Increase Reward and Final Answer Confidence Reward-we show that R-TAP-enhanced models consistently outperform conventional single-pass methods for both large language models (LLMs) and vision-language models (VLMs). Moreover, by analyzing the frequency of "Oops"-like expressions in model responses, we find that R-TAP-applied models exhibit significantly fewer self-reflective patterns, resulting in more stable and faster inference-time reasoning. We hope R-TAP pave the way evolving into efficient and elaborated methods to refine the reasoning processes of future AI.

==> figures/figure_llm_bench.tex <==
\makeatletter
\let\@oldmaketitle\@maketitle
\renewcommand{\@maketitle}{\@oldmaketitle
  \begin{center}
    \vspace{-3mm}
    \includegraphics[width=\textwidth]{figures/fig_llm_bench.pdf}
    \vspace{-5mm}
    \captionof{figure}{Overall accuracy (\%) of numerous large language models (LLMs) on five evaluation benchmarks—AIME25~\cite{patel2024aime}, HMMT Feb 25~\cite{hmmt}, OmniMath~\cite{gao2024omni}, GPQA~\cite{du2025supergpqa}, and LiveCodeBench~\cite{jain2024livecodebench}.}
    \label{fig:llm_bench}
  \end{center}
  \vspace{8mm} % Adjust this to control space between figure and abstract
}
\makeatother
% \twocolumn[{%
% \renewcommand\twocolumn[1][]{#1}%
% \maketitle % changed position of doing \maketitle
% \centering
% \vspace{-3mm}
% \includegraphics[width=\textwidth]{figures/fig_llm_bench.pdf}
% \vspace{-3mm}
% \captionof{figure}{Overall accuracy (\%) of numerous large language models (LLMs) on five evaluation benchmarks—AIME25~\cite{patel2024aime}, HMMT Feb 25~\cite{hmmt}, OmniMath~\cite{gao2024omni}, GPQA~\cite{du2025supergpqa}, and LiveCodeBench~\cite{jain2024livecodebench}.
% }
% \label{fig:llm_bench}
% \vspace{10mm}
% }]
% 
